Identifying Out-of-Distribution Samples in Real-Time for Safety-Critical 2D Object Detection with Margin Entropy Loss

Convolutional Neural Networks (CNNs) are nowadays often employed in vision-based perception stacks for safetycritical applications such as autonomous driving or Unmanned Aerial Vehicles (UAVs). Due to the safety requirements in those use cases, it is important to know the limitations of the CNN and, thus, to detect Out-of-Distribution (OOD) samples. In this work, we present an approach to enable OOD detection for 2D object detection by employing the margin entropy (ME) loss. The proposed method is easy to implement and can be applied to most existing object detection architectures. In addition, we introduce Separability as a metric for detecting OOD samples in object detection. We show that a CNN trained with the ME loss significantly outperforms OOD detection using standard confidence scores. At the same time, the runtime of the underlying object detection framework remains constant rendering the ME loss a powerful tool to enable OOD detection.

==> Chapters/plots/01_size_dependent.tex <==
\begin{tikzpicture}

    \definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
    \definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
    \definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

    \begin{axis}[
            height=0.4\textwidth,
            legend cell align={left},
            legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, nodes={scale=0.75, transform shape}},
            tick pos=left,
            width=0.95\textwidth,
            x grid style={white!69.0196078431373!black},
            xlabel={Maximum height [\si{\px}]},
            xmin=0, xmax=9,
            xtick style={color=black},
            y grid style={white!69.0196078431373!black},
            ylabel={Performance},
            ylabel style={yshift=-10pt},
            ytick style={color=black},
            xticklabels={
                    $0$,$<50$,$<100$,$<150$,$<200$,$<250$,$<300$,$<350$,$<400$,$<450$,$<500$
                }
        ]
        \addplot [thick, color0] table [x=x, y=separability,col sep=comma] {Chapters/plots/01_data.dat};
        \addlegendentry{$S$}
        \addplot [color1] table [x=x, y=ofs,col sep=comma] {Chapters/plots/01_data.dat};
        \addlegendentry{OFS}
        \addplot [color2] table [x=x, y=obs,col sep=comma] {Chapters/plots/01_data.dat};
        \addlegendentry{OBS}
    \end{axis}

\end{tikzpicture}

==> Chapters/plots/02_iop.tex <==

\begin{tikzpicture}

    \definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
    \definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
    \definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

    \begin{axis}[
            height=0.4\textwidth,
            legend cell align={left},
            legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, nodes={scale=0.75, transform shape}},
            tick pos=left,
            width=0.48\textwidth,
            x grid style={white!69.0196078431373!black},
            xlabel={Maximum height [\si{\px}]},
            xmin=0, xmax=9,
            xtick style={color=black},
            y grid style={white!69.0196078431373!black},
            ylabel={Performance},
            ytick style={color=black},
            ylabel style={yshift=-10pt},
            xticklabels={
                    $0$,$<50$,$<150$,$<250$,$<350$,$<450$,$<500$
                }
        ]
        \addplot [thick, color0] table [x=x, y=separability,col sep=comma] {Chapters/plots/01_data_iop.dat};
        \addlegendentry{$S$}
        \addplot [color1] table [x=x, y=ofs,col sep=comma] {Chapters/plots/01_data_iop.dat};
        \addlegendentry{OFS}
        \addplot [color2] table [x=x, y=obs,col sep=comma] {Chapters/plots/01_data_iop.dat};
        \addlegendentry{OBS}
    \end{axis}

\end{tikzpicture}

==> Chapters/plots/02_iop_diff.tex <==

\begin{tikzpicture}

    \definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
    \definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
    \definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

    \begin{axis}[
            height=0.4\textwidth,
            legend cell align={left},
            legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, nodes={scale=0.75, transform shape}},
            tick pos=left,
            width=0.48\textwidth,
            x grid style={white!69.0196078431373!black},
            xlabel={Maximum height [\si{\px}]},
            xmin=0, xmax=9,
            xtick style={color=black},
            y grid style={white!69.0196078431373!black},
            ylabel={Difference},
            ytick style={color=black},
            ylabel style={yshift=-10pt},
            xticklabels={
                    $0$,$<50$,$<150$,$<250$,$<350$,$<450$,$<500$
                }
        ]
        \addplot [thick, color0] table [x=x, y=separability,col sep=comma] {Chapters/plots/01_data_iop_diff.dat};
        \addlegendentry{$S$}
        \addplot [color1] table [x=x, y=ofs,col sep=comma] {Chapters/plots/01_data_iop_diff.dat};
        \addlegendentry{OFS}
        \addplot [color2] table [x=x, y=obs,col sep=comma] {Chapters/plots/01_data_iop_diff.dat};
        \addlegendentry{OBS}
    \end{axis}

\end{tikzpicture}

==> Chapters/plots/ablation_study.tex <==
\begin{tikzpicture}

    \definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
    \definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
    \definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

    \begin{axis}[
            height=0.4\textwidth,
            legend cell align={left},
            legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, nodes={scale=0.75, transform shape}},
            tick pos=left,
            width=0.95\textwidth,
            x grid style={white!69.0196078431373!black},
            xlabel={Margin},
            xmin=0, xmax=1,
            xtick style={color=black},
            y grid style={white!69.0196078431373!black},
            ylabel={Performance \newline (mAP/ Separability)},
            %ylabel style={yshift=-10pt},
            ytick style={color=black},
            xticklabels={
                    $0$,$0.05$,$0.1$,$0.5$,$1$
                }
        ]
        % \addplot [thick, color0] table [x=x, y=separability,col sep=comma] {};
        % \addlegendentry{$S$}
        % \addplot [color1] table [x=x, y=ofs,col sep=comma] {};
        % \addlegendentry{OFS}
        % \addplot [color2] table [x=x, y=obs,col sep=comma] {};
        % \addlegendentry{OBS}
    \end{axis}

\end{tikzpicture}

==> Chapters/results/97_details_results_me_loss.tex <==
\begin{table}[]
    \begin{tabular}{llllllll}
    \cline{1-1}
    \multicolumn{1}{|l|}{Class} & Images & Labels & P     & R      & F1     & mAP@.5 & mAP@.5:.95 \\ \cline{1-1}
    all                         & 3222   & 3998   & 0.611 & 0.333  & 0.361  & 0.356  & 0.248      \\
    Airborne                    & 3222   & 357    & 0.431 & 0.0616 & 0.108  & 0.0956 & 0.0497     \\
    Airplane                    & 3222   & 867    & 0.867 & 0.609  & 0.715  & 0.683  & 0.479      \\
    Bird                        & 3222   & 151    & 0.283 & 0.0199 & 0.0371 & 0.0219 & 0.0169     \\
    Drone                       & 3222   & 36     & 0.726 & 0.778  & 0.751  & 0.794  & 0.59       \\
    Flock                       & 3222   & 22     & 1     & 0      & 0      & 0      & 0          \\
    Helicopter                  & 3222   & 2565   & 0.968 & 0.865  & 0.913  & 0.901  & 0.599      \\
    ood                         & 3222   & 0      & 0     & 0      & 0      & 0      & 0         
    \end{tabular}
\end{table}

Since the OOD class has no samples in the ID training dataset (results presented above), it achieves an AP score of \num{0}. We account for this problem by calculating the mAP score without the OOD class. These values are given in section  4 of the related paper.

==> Chapters/results/98_details_results_baseline.tex <==
\begin{table}[]
    \begin{tabular}{llllllll}
    \cline{1-1}
    \multicolumn{1}{|l|}{Class} & Images & Labels & P      & R      & F1    & mAP@.5 & mAP@.5:.95 \\ \cline{1-1}
    all                         & 3222   & 3998   & 0.514  & 0.362  & 0.366 & 0.321  & 0.215      \\
    Airborne                    & 3222   & 357    & 0.192  & 0.157  & 0.173 & 0.0774 & 0.035      \\
    Airplane                    & 3222   & 867    & 0.686  & 0.637  & 0.66  & 0.611  & 0.417      \\
    Bird                        & 3222   & 151    & 0.0588 & 0.0927 & 0.072 & 0.0178 & 0.0118     \\
    Drone                       & 3222   & 36     & 0.757  & 0.777  & 0.767 & 0.666  & 0.478      \\
    Flock                       & 3222   & 22     & 1      & 0      & 0     & 0      & 0          \\
    Helicopter                  & 3222   & 2565   & 0.905  & 0.872  & 0.888 & 0.875  & 0.56       \\
    ood                         & 3222   & 0      & 0      & 0      & 0     & 0      & 0         
    \end{tabular}
\end{table}

Since the OOD class has no samples in the ID training dataset (results presented above), it achieves an AP score of \num{0}. We account for this problem by calculating the mAP score without the OOD class. These values are given in section  4 of the related paper.

==> eccv_workshop_uncertainty_ea/Chapters/1_intro.tex <==
\section{Introduction}
The development of UAVs strongly accelerated within the last decade through advances in robotics and artificial intelligence.
% While UAVs have been deployed in military use cases since the 20th century, the attention is shifting towards commercial applications in recent years.
% The autonomous operation of UAVs in civilian airspace provides a number of challenges for drone manufacturers, operators, and aviation agencies, among which collision avoidance is one of the most significant.
In order to mitigate collision risks, Detect-and-Avoid (DAA) systems are being developed to provide safe autonomy to UAVs by staying \emph{well clear} from other airborne traffic \cite{astmf3442}.
%
%While commercial airplanes rely on transponder-based systems such as the Traffic Alert and Collision Avoidance System (TCAS), they are not available on all classes of possible intruders.
%\todo{Source}
Similarly to perception stacks of other autonomous vehicles, computer vision has emerged as a mode of detecting and tracking other airspace participants.

CNNs have achieved state-of-the-art performance in computer vision tasks -- \eg semantic segmentation and object detection -- and have thus become the foundation of modern environment perception systems.
In the use case of detecting and avoiding other objects, vision-based DAA systems often employ 2D object detection CNN architectures such as Yolo \cite{redmon2016you} or SSD \cite{liu2016ssd}.
While neural networks in general have been deployed with great success, they typically do not provide self-evaluation with respect to their predictions \cite{jourdan_identication_2020}.
DAA systems are safety-critical components of UAVs, and it is, therefore, necessary that they actively self-identify their limitations as there may be no human pilot available as a fallback option \cite{CoDANN2,easa_ai_level1}.
Limitations include scene configurations or object classes that were not part of the training dataset of the neural networks.
This type of data is often referred to as \emph{Out-of-Distribution} (OOD) data in contrast to \emph{In-Distribution} (ID) data used during the training stage.
%Training datasets are finite and can thus not contain every possible situation a UAV might encounter \emph{in the wild}.
In the presence of OOD data, the desired behavior of the object detection system would be to express low confidence or high uncertainty for the detection but still identify relevant objects in contrast to the background.
An example for possible OOD data is shown in \autoref{fig:balloons}.
%While the vast majority of hot air balloons have a characteristic shape, there is a broad range of creative shapes that cannot be captured to full extend in the training data set for vision-based DAA systems.
The DAA system, however, must perceive all of those objects and initiate countermeasures to avoid potential collisions.

\begin{figure}[t]
    \centering
    % \includegraphics[width=0.30\columnwidth]{Chapters/imgs/hotairballoon.jpg}
    \includegraphics[width=0.29\columnwidth]{Chapters/imgs/emoji.jpg}
    %\includegraphics[width=0.16\textwidth]{Chapters/imgs/lok.jpg}
    %\includegraphics[width=0.16\textwidth]{Chapters/imgs/sekt.jpg}
    \includegraphics[width=0.29\columnwidth]{Chapters/imgs/cola}
    \includegraphics[width=0.29\columnwidth]{Chapters/imgs/schraubenzieher.jpg}
    \caption{Exemplary OOD hot air balloons.
        Most hot air balloons have a characteristic shape, while others have a rather creative design \cite{hot_air_ood}.
        % This variety of shapes probably won't be reflected in most training sets rendering some of those balloons as OOD objects.
    }
    \label{fig:balloons}
\end{figure}

Methods for uncertainty estimation and detection of OOD instances in CNNs often rely on sampling the network multiple times \eg, \cite{gal_dropout_2016,lakshminarayanan2017simple}, which is infeasible in computationally constrained environments such as small UAVs.
Thus, we present and evaluate a simple yet effective training strategy that can extend most existing object detection architectures with uncertainty estimation for OOD detection.
We exemplary extend the YoloX \cite{ge2021yolox} framework and evaluate the performance of the proposed method on a semi-synthetic aerial dataset.
We show that the OOD performance significantly exceeds the baseline performance while keeping the runtime of the detection system unchanged.
% We object detection network with the proposed method and evaluate the performance.

\bigbreak

\begin{comment}
This work provides the following main contributions:
\begin{enumerate}[label=\arabic*)]
    \item We propose a novel approach to learn uncertainty estimation for OOD detection in the setting of 2D object detection using an extended \emph{Margin-Entropy} (ME) loss function.
          Our approach only extends the training strategy and therefore does not require any changes to the network architecture.
          In particular, it does not increase the inference runtime.
    \item We propose a novel extension to the confusion matrix and a derived \emph{Separability} metric to allow for the practical evaluation of OOD performance in safety critical use cases.
    \item We exemplary extend the YoloX \cite{ge2021yolox} object detection network with the proposed method and evaluate the performance on a semi-synthetic dataset.
\end{enumerate}

The remainder of the paper is structured as follows:
\Cref{sec:related_work} introduces and structures existing approaches for OOD in deep learning-based object detection.
In \Cref{sec:model}, the proposed novel method for OOD in object detection based on the ME loss as well as the implemented baselines are introduced.
The performance of the proposed method is subsequently evaluated and compared \textcolor{red}{using existing and newly proposed metrics} in \Cref{sec:results}.
Finally, \Cref{sec:conclusion} provides a conclusion of the findings as well as the identified potentials for future work.

\textcolor{red}{
    \textbf{TODO / TO Check:}
    \begin{enumerate}
        \item Data generation should be introduced in experiments section-> One more sentencte in Sec 4.1
    \end{enumerate}
}

\end{comment}

==> eccv_workshop_uncertainty_ea/Chapters/2_related_work.tex <==
\section{Related Work}
Out-of-distribution detection is a popular research stream for various computer vision tasks, such as image classification \cite{hendrycks_baseline_2018,lee_simple_2018,liang_enhancing_2020} and semantic segmentation \cite{chan2021entropy,kendall2015bayesian,jourdan_identication_2020}.
More recently, the topic is gaining traction in object detection research as well \cite{dhamija2020overlooked}.
Concerning the overall methodology and runtime, we divide related OOD approaches for object detection into \emph{sampling} methods and \emph{sampling free} methods.

Sampling methods often rely on test-time activation of dropout \cite{srivastava2014dropout} layers to approximate inference of a Bayesian Neural Network (BNN).
This concept was first introduced as Monte-Carlo (MC) Dropout in \cite{gal2015bayesian} and consequently applied to computer vision tasks such as semantic segmentation \cite{kendall2015bayesian}.
\cite{miller2018dropout} applies MC Dropout to the SSD \cite{liu2016ssd} object detection architecture.
Box detections of multiple forward passes are grouped and aggregated by Intersection-over-Union (IoU) overlap.
Consequently, uncertainties with regard to position regression and classification are derived from these samples.
\cite{kraus_uncertainty_2019} introduced Bayesian YoloV3.
In addition to MC Dropout, variances are predicted for the location parameters of the regressed bounding boxes.
\cite{harakeh2020bayesod} replaces the Non-Maximum Suppression (NMS) with bayesian inference for enhanced uncertainty estimation.
Lastly, \cite{deepshikha2021monte} proposed the use of Dropblock \cite{ghiasi2018dropblock} instead of dropout for obtaining the BNN samples.
As an alternative to MC dropout sampling, deep ensembles may be used to obtain multiple detection samples for a given image.
Deep ensembles have been proposed for OOD in image classification by \cite{lakshminarayanan2017simple}.
\cite{lyu2020probabilistic} uses ensemble samples for uncertainty estimation in object detection networks.

Sampling methods for OOD are not suitable for the use case of UAV DAA systems as multiple forward passes increase the computation time by orders of magnitude.
This renders real-time detection with high-resolution cameras infeasible on low-power hardware usually found in drones.

Sampling-free methods for OOD in object detection are considerably rarer in literature.
\cite{joseph2021towards} proposed using energy-based models on the output logits of object detection networks to discriminate between ID and OOD samples combined with a form of temperature scaling.
\cite{schubert2021metadetect} uses a post-processing method for uncertainty estimation of object detection networks.
A meta classification approach is employed that generates confidence based on box parameters and metrics derived from boxes in the NMS.

==> eccv_workshop_uncertainty_ea/Chapters/3_model.tex <==
\section{Model}
\label{sec:model}
%\textcolor{red}{Todo Yannik}
To enable OOD detection in the setting of 2D object detection with our proposed approach, only minimal changes in the loss function are required.
Particularly, it does not require any adjustments in the network architecture.
It can therefore easily be included in any modern 2D object detection framework like Faster R-CNN \cite{girshick2015fast,ren2015faster}, SSD \cite{liu2016ssd}, and the various Yolo variants \cite{redmon2016you,redmon2017yolo9000,redmon2018yolov3,ge2021yolox}.
As the architecture of the final CNN remains the same, the initial runtime of the underlying object detection framework is preserved.
%We start by using the softmax function to obtain pseudo probabilities as a the baseline method \cite{hendrycks_baseline_2018}.
%We further explain the adaption of this method, its limitations, and \emph{margin entropy loss} as a solution to the baseline's problems.

%In this section we explore the changes, applied to our machine learning model to enable and then to further improve Out-Of-Distribution detection. First, we show, how the softmax function can be adapted as a na\"ive baseline to the problem. Then, we introduce the "Margin-Entropy-Loss" as an approach to make the models softmax scores better reflect the expected confidence. Third, we give an introduction to the metrics, used to rate the models OOD-performance. Finally, we present the generation pipeline for Out-Of-Distribution samples, used as a base of this work.

\begin{comment}
\subsection{Foreground, Background, ID, and OOD}
In inference, we are dealing with foreground (FG) and background (BG) objects.
Foreground objects are all objects in the image, that are relevant to the detection task.
Background objects on the other hand are known but irrelevant.
In our use case, such an object could be a cloud.
We can further divide the objects regarding their presence in the training data. ID objects are part of the training distribution as a foreground ($ID_{FG}$) or as a background object($ID_{BG}$).
All objects, not related to the training data, but important for the classification task, are referred to as OOD.
\todo{ID/OOD definition duplicates section 1}
\end{comment}


\subsection{Confidence Thresholding}

Multiple approaches utilize the model's raw confidence outputs computed by sigmoid or softmax activations as a base for uncertainty quantification in classification tasks \cite{schwaiger_is_2020,hendrycks_baseline_2018}.
In pure image classification, an image is either ID, \ie it has been part of the training, or OOD.
During training, the CNN is trained to best possibly recognize ID properties.
The more ID properties a CNN can detect within an image, the more confident it is with the final classification.
As a result, we expect that images with known objects, patterns, or structures have higher predicted confidence $\max_i p_i(x)$ than those with unknown ones \ie,  OOD.
Thus, it is a natural choice to distinguish between ID and OOD based on the confidence of the classification.
In object detection, however, an image may contain multiple instances of both ID -- containing both Foreground (FG) objects and Background (BG) -- and OOD objects.
To account for the presence of multiple objects and to distinguish between known foreground (ID\textsubscript{FG}), known background (ID\textsubscript{BG}), and unknown OOD objects, we impose two thresholds based on the confidence, \ie softmax score.
An illustration of the thresholds is given in \autoref{fig:thresholds}.

\begin{figure}[t]
  \definecolor{dblue}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
  \definecolor{dorange}{rgb}{1,0.498039215686275,0.0549019607843137}
  \definecolor{dgreen}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
  \centering
  \begin{tikzpicture}
    \draw [-stealth](0,0) -- (8,0);
    \draw (0,+3pt) -- (0,-3pt) node[below] {0};
    \draw (3,+3pt) -- (3,-3pt) node[below] {$t_{\text{ID}_\text{BG}}$};
    \draw (5,+3pt) -- (5,-3pt) node[below] {$t_{\text{ID}_\text{FG}}$};
    \draw (7.5,+3pt) -- (7.5,-3pt) node[below] {1};
    \node[mark size=3pt,color=dgreen] at (2,0) {\pgfuseplotmark{*}};
    \node[mark size=3pt,color=dorange] at (3.5,0) {\pgfuseplotmark{*}};
    \node[mark size=3pt,color=dblue] at (7.2,0) {\pgfuseplotmark{*}};
    \node[anchor=north west, xshift=-6pt, yshift=-13pt] at (0,0) {Foreground Confidence};
  \end{tikzpicture}
  \caption{Visualization of the thresholds over the confidence value.
    A prediction represented by the \textbf{\textcolor{dgreen}{green}} circle is treated as a background object.
    In contrast, predictions represented by \textbf{\textcolor{dorange}{orange}} and \textbf{\textcolor{dblue}{blue}} circles are both treated as \emph{actual} out-of-distribution and foreground objects, respectively.}
  \label{fig:thresholds}
\end{figure}

We can easily employ a threshold-based classifier to assign a final category $C$ of a prediction of the CNN such that
\begin{equation}
  C=
  \left\{
  \begin{array}{ll}
    \text{ID}_{\text{BG}} & \text{if } 0 \le \max_i p_i(x) < t_{\text{ID}_\text{BG}} ,                       \\
    \text{OOD}            & \text{if } t_{\text{ID}_\text{BG}} \le \max_i p_i(x)  < t_{\text{ID}_\text{FG}}, \\
    \text{ID}_{\text{FG}} & \text{if } t_{\text{ID}_\text{FG}} \le \max_i p_i(x)  < 1.
  \end{array}
  \right.
  \label{eq:func_distributions}
\end{equation}

\subsection{Margin Entropy Loss}
CNNs commonly tend to be overconfident \cite{nguyen_deep_2015}.
Therefore, predictions are also overconfident for OOD samples \cite{gal_dropout_2016}.
As a result, the distributions for both ID and OOD samples are overlapping and we can not easily separate them through the application of $t_{\text{ID}_\text{BG}}$ and $t_{\text{ID}_\text{FG}}$.
Due to this problem, we expect confidence thresholding on onchanged network outputs to not perform sufficiently well in distinguishing ID from OOD samples.
The \emph{Margin Entropy} (ME) loss term introduced in \cite{vyas2018out} as an approach to tackle the problem of overconfidence.
% First, we define the goals for this loss function.
It has already been researched in \cite{jourdan_identication_2020} for semantic segmentation and has proven to effectively detect OOD pixels.
The ME loss is mathematically defined to be high in those cases, where the model estimates high confidence for OOD samples.
In return, it shall not affect the training of ID samples.
We, therefore, define it to be $0$ for all images with ID samples only.
As a proxy for the uncertainty of the model, we employ the Shannon entropy $H$ for discrete probability distributions with class confidences $p_i(x)$ for a given sample $x$ and $N_C$ being the total number of classes as
\begin{equation}
  H(x) = - \sum_{i = 1}^{N_C} p_i(x) \log p_i(x).
  \label{eq:entropy}
\end{equation}
A uniform distribution of the class confidences cause the entropy to be at its maximum, while in contrast, the entropy is minimal if the confidence is concentrated in a single class. We define the \emph{Margin Entropy} loss term as

\begin{equation}
  \mathcal{L}_{me} = \max{(m+\bar{H}_{\text{ID}_{\text{FG}}}-\bar{H}_{\text{OOD}}, 0)}
\end{equation}
where $\bar{H}_{\text{ID}_{\text{FG}}}$ denotes the average entropy on FG samples and $\bar{H}_\text{OOD}$ denotes the average entropy on OOD samples.
$m$ is a hyperparameter that controls the \emph{margin} between both entropies.
According to \cite{vyas2018out}, the application of a margin in contrast to entropy maximization prevents overfitting on the OOD areas and reduces negative effects on the original task.
% We will now transfer the idea to object detection.

In 2D object detection, the overall loss $\mathcal{L}$ comprises a localization loss $\mathcal{L}_\text{loc}$ and the classification loss $\mathcal{L}_\text{cls}$.
Finally, ME loss $\mathcal{L}_{\text{me}}$ is included as an additional loss such that the overall loss $\mathcal{L}$ calculates as
\begin{align}
  \mathcal{L}=\mathcal{L}_{\text{loc}}+\beta_1 \mathcal{L}_{\text{cls}} + \beta_2 \mathcal{L}_{\text{me}}.
\end{align}
$\beta_1$ and $\beta_2$ are used to control the magnitude of the loss components.



%https://openaccess.thecvf.com/content_ECCV_2018/papers/Apoorv_Vyas_Out-of-Distribution_Detection_Using_ECCV_2018_paper.pdf

\begin{comment}
\subsection{Generation of Out-Of-Distribution Samples}
\label{text:generation}
%\textcolor{red}{Todo Yannik}

OOD samples are required in the training and in the evaluation step of the pipeline.
We, therefore, need images with unknown objects that are still relevant to the detection task.
Since such images are not available, we created them ourselves from CAD models. We chose these models in a way that similar objects are not present in the training data.
We present the procedure in \autoref{fig:data_generation}.
First, CAD models for OOD objects were chosen.
Even though we don't expect overfitting on OOD samples in the training process, we chose different models for training and validation.

\begin{figure}[t]
  \centering
  \tikzstyle{ressource} = [rectangle, rounded corners, minimum width=3.5cm, minimum height=1cm,text centered, draw=black, fill=green!20]
  \tikzstyle{process} = [rectangle, minimum width=3.5cm, minimum height=1cm, text centered, draw=black, fill=gray!30]
  \tikzstyle{arrow} = [thick,->,>=stealth]
  \tikzstyle{final} = [rectangle, minimum width=3.5cm, minimum height=1cm, text centered, draw=black, fill=red!30]
  \tikzstyle{arrow} = [thick,->,>=stealth]

  \begin{tikzpicture}[node distance=1.5cm]
    \node (cad) [ressource] {CAD Model};
    \node (path) [ressource, below of=cad] {Flight Path};
    \node (properties) [ressource, below of=path] {Model Properties};

    \node (blender) [process, right of=path, xshift=2.7 cm] {Blender};
    \node (merger) [process, right of=blender, xshift=2.7 cm] {Frame Merger};

    \node (back) [ressource, above of=merger] {Scene Background};
    \node (res) [final, below of=merger] {Merged Image};

    \draw [arrow] (cad) -| (blender);
    \draw [arrow] (path) -- (blender);
    \draw [arrow] (properties) -| (blender);
    \draw [arrow] (blender) -- (merger);
    \draw [arrow] (back) -- (merger);
    \draw [arrow] (merger) -- (res);
  \end{tikzpicture}
  \caption{Pipeline for the generation of OOD samples. We combine CAD model, flight path, model properties and, a background scene into one image, containing an OOD object. This image can then be used for training the network.}
  \label{fig:data_generation}
\end{figure}

%Hier eine Matrix mit den renderings einbauen
\begin{figure}
  \centering
  \begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{graph1}
    \caption{$y=x$}
    \label{fig:y equals x}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{graph2}
    \caption{$y=3sinx$}
    \label{fig:three sin x}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{graph3}
    \caption{$y=5/x$}
    \label{fig:five over x}
  \end{subfigure}
  \caption{Three simple graphs}
  \label{fig:three graphs}
\end{figure}

We can then use the model itself, recorded or random flight paths, and model properties such as its common spacial orientations to create configurations for the 3D rendering software \emph{Blender}.
We additionally choose random body colors to ensure maximum of versatility. We then place the objects on previously recorded flight paths or on fixed positions with random orientations.
It is highly relevant for the second case to limit the number of poses.
A hot air balloon could for example not be flipped upside down.
We, therefore, define a set of model properties.
Further, a set of scene backgrounds is chosen.
These are preferably empty images to prevent renderings from occluding ID objects.
Merging is performed by using the following equation.

\begin{equation}
  \textbf{M} = \textbf{B}*(255-\textbf{R}_\text{a})+\textbf{R}_\text{g} \textbf{R}_\text{a}
\end{equation}

\noindent
$\textbf{M}$ denotes the merged image and $\textbf{B}$ the base image.
We further split the rendered image $\textbf{R}$ into its alpha channel $\textbf{R}_\text{a}$ and its grayscale component $\textbf{R}_\text{g}$.
All images are applied as \emph{uint8} data type.

\end{comment}


==> eccv_workshop_uncertainty_ea/Chapters/4_experiments.tex <==
\section{Experiments}
\label{sec:results}
%\textcolor{red}{Todo Yannik}

\subsection{Dataset}
In our experiments, we use a subset of the \emph{Amazon AOT Dataset} \cite{amazon_aot}, containing \num{12247} objects on \num{10071} images as training data for the network.
Additionally, we created \num{692} photorealistic renderings of \num{5} 3D models on \num{144} images for training treated as OOD samples.
Each rendered image is merged with an image from the actual Amazon AOT Dataset during training to provide a wider range of configurations.
We validated the method on a set containing \num{332} rendered OOD objects based on \num{3} different 3D models and \num{3998} ID objects on \num{3222} images.
The 3D models were exclusively used in either the training or the validation dataset.

\subsection{Experimental Setup}
\label{sec:setup}
For training and evaluation, we extend the state-of-the-art YoloX \cite{ge2021yolox} object detection framework with the ME loss. We compare the OOD detection performance to the unchanged network output trained with the standard loss function.
%
\begin{comment}
We additionally chose the values below for the margin $m$ and trained one model each to conduct a sensitivity study.

\begin{equation}
    m = \{0.05, 0.1, 0.5, 1\}
\end{equation}
\end{comment}
%
%
%- Welche Learning rate (David fragen wegen strategie!)
%
\subsection{Metrics}
%\textcolor{red}{examples for OBS, OFS, S. Give the range of the metric, eg 0 to 1, 1 is better.}
In a typical object detection setting, metrics like Average Precision (AP) and Mean Average Precision (mAP) are used to quantify the performance of the underlying detection framework.
These metrics comprise the number of True Positive (TP), False Positive (FP), and False Negative (FP) predictions.
%Those metrics build upon Precision and Recall metrics, which in turn require an assigment of the predicted objects as being either True Positive (TP), False Positive (FP), or False Negatives (FN).
%To either accept or decline a prediction, an auxiliary metric like IoU is employed to quantify the overlap between a predicted and a GT object.
%Eventually, a prediction is accepted as TP if it exceeds an IoU threshold of typically \num{0.5} or \num{0.7} \cite{everingham2010pascal,geiger2012we,gahlert2020cityscapes}.
%
\begin{comment}
\textcolor{red}{
    Based on these assignments, the standard performance metrics Precision and Recall can be calculated as
    \begin{align}
        \text{Precision} & = \frac {\text{TP}} {\text{TP} + \text{FP}}  \\
        \text{Recall}    & = \frac {\text{TP}} {\text{TP} + \text{FN}}.
    \end{align}
}
\end{comment}
%
Besides AP, Liang \etal introduced additional metrics to assess the OOD detection performance \cite{liang_enhancing_2020}.
These metrics include FPR@\SI{95}{\percent} TPR and AUROC.
The definition of both metrics include the calculation of the False Positive Rate (FPR) defined as $\text{FPR} = \tfrac{\text{FP}} {\text{FP} + \text{TN}}$.
In particular, this metric uses the total number of True Negatives (TN).
Current state-of-the-art object detection frameworks employ a set of intial proposals called \emph{anchor} or \emph{prior boxes} \cite{liu2016ssd,redmon2016you}.
The number of those boxes scales with the image size and might reach several \num{10}k boxes per image.
As the number of \emph{real} objects, however, is typically small compared to the number of anchor or prior boxes, the number of TN will be close to the total number of those initial boxes.
This leads to $\text{FPR} \approx 0$ in most object detection frameworks even at small confidence thresholds and in particular, can change depending on the image size.
As a result, metrics that comprise the number of TN are highly influenced by the experimental setup and do not properly assess the OOD performance in object detection.

We propose to extend the confusion matrix to account for OOD objects and derive a novel \emph{Separability} metric to assess the OOD performance.

\subsubsection{Extended OOD Confusion Matrix}
The binary assignment of being either FG or BG does not specifically reflect the OOD setting as OOD objects are \emph{in between} FG and BG.
To account for those objects, we propose to add OOD as a meta-class to the confusion matrix.
This extended confusion matrix is shown in \autoref{tab:confmatrix}.

\begin{table}[t]
    \caption{Proposed confusion matrix that takes into account the OOD objects.}
    \label{tab:confmatrix}
    \centering
    \begin{tabular}{ccccc}
                                            &                                   & \multicolumn{3}{c}{\textbf{Actual}}                                                                  \\
                                            &                                   & \textbf{BG}                         & \textbf{OOD}        & \textbf{FG}                              \\\cline{3-5}
        \multirow{3}{*}{\textbf{Predicted}} & \multicolumn{1}{c|}{\textbf{BG}}  & TN                                  & FN\textsubscript{O} & \multicolumn{1}{c|}{FN}                  \\
                                            & \multicolumn{1}{c|}{\textbf{OOD}} & FO\textsubscript{N}                 & TO                  & \multicolumn{1}{c|}{FO\textsubscript{P}} \\
                                            & \multicolumn{1}{c|}{\textbf{FG}}  & FP                                  & FP\textsubscript{O} & \multicolumn{1}{c|}{TP}                  \\ \cline{3-5}
    \end{tabular}
\end{table}

We define \emph{True OOD} (TO) as actual OOD objects that have been assigned as OOD.
Furthermore, we refer to OOD objects that have been falsely assigned as FG as FP\textsubscript{O} and in return FG objects that are treated as OOD objects as \emph{False OOD/Foreground} (FO\textsubscript{P}).
Following this naming convention, we define the analogous metrics for BG objects.

\subsubsection{Separability}
To assess the quality of OOD detection within the scope of 2D object detection, we propse a novel metric called \emph{Separability} which builds upon the extended confusion matrix defined above.
Its core idea is to quantify the ability of the network to separate between FG, BG and OOD objects. It comprises two auxiliary metrics called \emph{OOD-Background Separability} (OBS) and \emph{OOD-Foreground Separability} (OFS) with each metric particularly assessing the ability to distinguish between FG or BG and OOD:
\begin{align}
    \text{OBS} & = \frac {\text{TO}} {\text{TO} + \text{FN\textsubscript{O}} + \text{FO\textsubscript{N}}}  \\
    \text{OFS} & = \frac {\text{TO}} {\text{TO} + \text{FP\textsubscript{O}} + \text{FO\textsubscript{P}}}.
\end{align}
Both OBS and OFS are $\in [0,1]$ with higher numbers representing a better ability to separate between BG and OOD, and FG and OOD.
Finally, we calculate \emph{Separability} $S(\beta)$ as
\begin{align}
    S(\beta) & = (1 + \beta^2) \cdot \frac {\text{OBS} \cdot \text{OFS}} {(\beta ^2 \cdot \text{OBS}) + \text{OFS}}.
\end{align}
Similar to OBS and OFS, $S \in [0,1]$ with higher values representing a better overall separability.
By using the parameter $\beta$ we can weight the impact of both OBS and OFS.
In our experiments, however, we use $\beta = 1$.


Contrary to the standard metrics for object detection AP and mAP, the Separability is not integrated over multiple confidence thresholds.
Instead, it assesses the model performance \emph{as is} if deployed to a productive system like autonomous drones or automated cars.
In those use cases, typically a fixed confidence threshold is chosen to allow an object to be spawned.


\subsection{Results}
We evaluate both the baseline confidences, trained with the standard cross-entropy loss, as well as the proposed method using the ME loss according to the experimental setup described in \autoref{sec:setup}.
The results are shown in \autoref{tab:results}.
%Qualitative results are shown in \autoref{fig:qualitative}.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.47\columnwidth]{Chapters/results/small_crop.png}
%     \includegraphics[width=0.47\columnwidth]{Chapters/results/medium_crop.png}
%     %\quad
%     %\subfloat[Large OOD object, height = \SI{277}{\px}.]{\includegraphics[width=0.3\textwidth]{Chapters/results/large_crop.png} \label{fig:largecrop}}
%     \caption{Qualitative results for 2 rendered objects of different size.}
%     \label{fig:qualitative}
% \end{figure}
%
\input{Chapters/results/99_results_table.tex}
%
The proposed ME loss approach outperforms the na\"ive baseline by \SI{129}{\percent} by means of separability $S$.
At the same time, the individual separability between OOD and BG and FG are \num{0.431} and \num{0.556}, respectively.
Thus, ME loss proves to significantly improve OOD detection in the scope of 2D object detection.

\begin{comment}
\subsection{Ablation Studies}

\subsubsection{In-Depth and Failure Case Analysis}
To better understand the boundaries and possible edge cases of the proposed ME loss approach, we conduct an in-depth and failure case analysis.

The challenge in object detection is twofold: On one hand, the CNN needs to be able to properly classify the object.
On the other hand, it simultaneously needs to learn how to perfectly localize the object by means of a 2D bounding box.
Thus, there are two potential sources of error that might prevent the object detection framework from perfectly detecting OOD objects.
In addition, previous studies have studied the complexity of detecting small objects \cite{fu2017dssd,li2017perceptual,cao2018feature}.

We, therefore, break the performance of the proposed ME loss down to different sizes of the objects and analyze the ability to properly classify and localize the objects.

The results are shown in \autoref{fig:iou_sizes}.

\begin{figure}[t]
    \centering
    \input{Chapters/plots/01_size_dependent.tex}
    \caption{Separability $S$, OFS, and OBS for different sized objects. For larger objects, the performance decreases.}
    \label{fig:iou_sizes}
\end{figure}

We find that both small as well as big object have a separability below the average.
For small objects, this effect can be traced back to the overall complexity of small object detection caused by the small receptive field.
The smaller the receptive field, the less information is available for the CNN.
For large objects, however, the degradation is caused by the breakup of the object into smaller predictions.
An example is shown in \autoref{fig:breakup}.

\begin{figure}[t]
    \centering
    \subfloat[Small OOD object, height = \SI{19}{\px}.]{\includegraphics[width=0.3\textwidth]{Chapters/results/small_crop.png}}
    \quad
    \subfloat[Medium OOD object, height = \SI{80}{\px}.]{\includegraphics[width=0.3\textwidth]{Chapters/results/medium_crop.png}}
    \quad
    \subfloat[Large OOD object, height = \SI{277}{\px}.]{\includegraphics[width=0.3\textwidth]{Chapters/results/large_crop.png} \label{fig:largecrop}}
    \quad
    \caption{Exemplary output for different sizes of OOD objects. Large objects tend to breakup into smaller predictions.}
    \label{fig:breakup}
\end{figure}

This disintegration naturally deteriorates the separability metrics as those smaller predictions are considered as FO\textsubscript{N}, while the actual object itself counts as a FN\textsubscript{O}.

In some use cases, however, it might be sufficient to know that there \emph{is} an OOD object instead of requiring an acurate localization within the image.
To consider and evaluate those cases, we need to relax the requirement of an IoU of \num{0.5} to assign a prediction as TP for OOD objects.
Instead, we use IoU as an auxiliary metric for FG objects, while using Intersection-over-Prediction (IoP) for OOD objects.
IoP between a predicted $p$ and a Ground Truth (GT) bounding box $g$ is defined as
\begin{align}
    \text{IoP}(p,g) = \frac {I(p,g) }{A(p)}
\end{align}
with $I(p,g)$ being the intersection between both boxes and $A(p)$ denoting the area of the predicted bounding box.
It measures the fraction of the predicted bounding box that overlaps with the actual GT box.
In cases like Figure \ref{fig:largecrop} the predicted bounding boxes are completely overlapping with the GT box and would thus be assigned as a correct prediction.

The results of the size-dependent analsysis is shown in \autoref{fig:iop}.
All three performance metrics yield better results for large object using IoP instead of IoU.
This verifies the assumption that the decreased performance can be traced back to the disintegrating of large objects.
In return, it proves that the classification of the OOD objects works well even for large objects.
Thus, our approach gives reasonable results even for large objects if the use case only requires the knowledge about the presence of an OOD object rather than the accurate localization.

\begin{figure}[t]
    \centering
    \subfloat[][Performance using IoP to match OOD objects.]{\input{Chapters/plots/02_iop.tex}}
    \quad
    \subfloat[][Difference to IoU based matching.]{\input{Chapters/plots/02_iop_diff.tex}}
    \caption{Separability $S$, OFS, and OBS for different sized objects using IoP as matching strategy. For larger objects, IoP yields better results.}
    \label{fig:iop}
\end{figure}




\subsubsection{Sensitivity Study}

We evaluated four values for the hyperparameter $m$ to approximate a suited configuration for our dataset.
The best OOD detection perforamance was achieved when applying  a margin of $m=\textcolor{red}{\num{0.1}}$.
It should be noted, that we aren't able to check for correlation of the optimal margin with the dataset.
We, therefore, recommend the reader to also run sensitivity studies to achieve the best performance of the presented method.

\begin{figure}[t]
    \centering
    \input{Chapters/plots/ablation_study.tex}
    \caption{Results for the sensitivity study. Separability rises monotinicaly with an increasing margin. mAP on the other hand decreases from a value of \textcolor{red}{X} onwards.}
    \label{fig:sens_study}
\end{figure}
\end{comment}


%\begin{comment}
\begin{figure}[t]
    \centering
    \subfloat[][Baseline]{\tikzBaselinePDF} \\
    \subfloat[][Margin Entropy Loss]{\tikzMElossPDF}
    \caption{Comparison of the confidence distribution after training with the baseline method (a) and the ME loss (b). We achieve a significantly better separation in (b) between all three distributions.}
    \label{fig:resDists}
\end{figure}
%\end{comment}

\begin{comment}

\subsection{Diagram Playground}
\textcolor{red}{In distribution: Summe aus background und foreground}
\subsubsection{Na\"ive Baseline: Softmax and Threshold}


\begin{figure}[!ht]
    \centering
    \tikzBaselinePDF
    \caption{Visualization of ID, OOD and Background distributions.}
\end{figure}

\end{comment}

\begin{comment}
\subsubsection{Marginal Entropy Loss}

\begin{figure}[!ht]
    \centering
    \tikzMElossPDF
    \caption{Visualization of ID, OOD and Background distributions.}
\end{figure}

\begin{table}
    \centering
    \tabMEloss
    \caption{ME Loss table.}
\end{table}

\end{comment}

==> eccv_workshop_uncertainty_ea/Chapters/5_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this work, we tackled the problem of OOD detection in the scope of 2D object detection.
To this end, we proposed to extend the overall loss function by an additional Margin Entropy loss.
In addition, we introduced the Separability metric to assess the ability of a network to distinguish between Foreground, Background, and OOD.
%
We evaluated the proposed ME loss on the Amazon AOT dataset \cite{amazon_aot}. The ME loss outperforms the na\"ive baseline by \SI{129}{\percent} by means of Separability. Furthermore, the pure 2D object detection performance is not degraded.
%
The proposed loss can be included in any modern object detection framework such as Faster R-CNN \cite{girshick2015fast,ren2015faster}, SSD \cite{liu2016ssd} and the various Yolo variants \cite{redmon2016you,redmon2017yolo9000,redmon2018yolov3,ge2021yolox}.
Compared to other methods like Ensembles or MC Dropout, it does not require multiple inference per image and in return, it is able to retain the inference speed of the underlying object detection framework.
Thus, the proposed loss proves to be a suitable extension to enable OOD detection for 2D object detection in time and safety-critical applications.

==> eccv_workshop_uncertainty_ea/Chapters/plots/01_size_dependent.tex <==
\begin{tikzpicture}

    \definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
    \definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
    \definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

    \begin{axis}[
            height=0.4\textwidth,
            legend cell align={left},
            legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, nodes={scale=0.75, transform shape}},
            tick pos=left,
            width=0.95\textwidth,
            x grid style={white!69.0196078431373!black},
            xlabel={Maximum height [\si{\px}]},
            xmin=0, xmax=9,
            xtick style={color=black},
            y grid style={white!69.0196078431373!black},
            ylabel={Performance},
            ylabel style={yshift=-10pt},
            ytick style={color=black},
            xticklabels={
                    $0$,$<50$,$<100$,$<150$,$<200$,$<250$,$<300$,$<350$,$<400$,$<450$,$<500$
                }
        ]
        \addplot [thick, color0] table [x=x, y=separability,col sep=comma] {Chapters/plots/01_data.dat};
        \addlegendentry{$S$}
        \addplot [color1] table [x=x, y=ofs,col sep=comma] {Chapters/plots/01_data.dat};
        \addlegendentry{OFS}
        \addplot [color2] table [x=x, y=obs,col sep=comma] {Chapters/plots/01_data.dat};
        \addlegendentry{OBS}
    \end{axis}

\end{tikzpicture}

==> eccv_workshop_uncertainty_ea/Chapters/plots/02_iop.tex <==

\begin{tikzpicture}

    \definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
    \definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
    \definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

    \begin{axis}[
            height=0.4\textwidth,
            legend cell align={left},
            legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, nodes={scale=0.75, transform shape}},
            tick pos=left,
            width=0.48\textwidth,
            x grid style={white!69.0196078431373!black},
            xlabel={Maximum height [\si{\px}]},
            xmin=0, xmax=9,
            xtick style={color=black},
            y grid style={white!69.0196078431373!black},
            ylabel={Performance},
            ytick style={color=black},
            ylabel style={yshift=-10pt},
            xticklabels={
                    $0$,$<50$,$<150$,$<250$,$<350$,$<450$,$<500$
                }
        ]
        \addplot [thick, color0] table [x=x, y=separability,col sep=comma] {Chapters/plots/01_data_iop.dat};
        \addlegendentry{$S$}
        \addplot [color1] table [x=x, y=ofs,col sep=comma] {Chapters/plots/01_data_iop.dat};
        \addlegendentry{OFS}
        \addplot [color2] table [x=x, y=obs,col sep=comma] {Chapters/plots/01_data_iop.dat};
        \addlegendentry{OBS}
    \end{axis}

\end{tikzpicture}

==> eccv_workshop_uncertainty_ea/Chapters/plots/02_iop_diff.tex <==

\begin{tikzpicture}

    \definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
    \definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
    \definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

    \begin{axis}[
            height=0.4\textwidth,
            legend cell align={left},
            legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, nodes={scale=0.75, transform shape}},
            tick pos=left,
            width=0.48\textwidth,
            x grid style={white!69.0196078431373!black},
            xlabel={Maximum height [\si{\px}]},
            xmin=0, xmax=9,
            xtick style={color=black},
            y grid style={white!69.0196078431373!black},
            ylabel={Difference},
            ytick style={color=black},
            ylabel style={yshift=-10pt},
            xticklabels={
                    $0$,$<50$,$<150$,$<250$,$<350$,$<450$,$<500$
                }
        ]
        \addplot [thick, color0] table [x=x, y=separability,col sep=comma] {Chapters/plots/01_data_iop_diff.dat};
        \addlegendentry{$S$}
        \addplot [color1] table [x=x, y=ofs,col sep=comma] {Chapters/plots/01_data_iop_diff.dat};
        \addlegendentry{OFS}
        \addplot [color2] table [x=x, y=obs,col sep=comma] {Chapters/plots/01_data_iop_diff.dat};
        \addlegendentry{OBS}
    \end{axis}

\end{tikzpicture}

==> eccv_workshop_uncertainty_ea/Chapters/plots/ablation_study.tex <==
\begin{tikzpicture}

    \definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
    \definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
    \definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

    \begin{axis}[
            height=0.4\textwidth,
            legend cell align={left},
            legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, nodes={scale=0.75, transform shape}},
            tick pos=left,
            width=0.95\textwidth,
            x grid style={white!69.0196078431373!black},
            xlabel={Margin},
            xmin=0, xmax=1,
            xtick style={color=black},
            y grid style={white!69.0196078431373!black},
            ylabel={Performance \newline (mAP/ Separability)},
            %ylabel style={yshift=-10pt},
            ytick style={color=black},
            xticklabels={
                    $0$,$0.05$,$0.1$,$0.5$,$1$
                }
        ]
        % \addplot [thick, color0] table [x=x, y=separability,col sep=comma] {};
        % \addlegendentry{$S$}
        % \addplot [color1] table [x=x, y=ofs,col sep=comma] {};
        % \addlegendentry{OFS}
        % \addplot [color2] table [x=x, y=obs,col sep=comma] {};
        % \addlegendentry{OBS}
    \end{axis}

\end{tikzpicture}

==> eccv_workshop_uncertainty_ea/Chapters/results/97_details_results_me_loss.tex <==
\begin{table}[]
    \begin{tabular}{llllllll}
    \cline{1-1}
    \multicolumn{1}{|l|}{Class} & Images & Labels & P     & R      & F1     & mAP@.5 & mAP@.5:.95 \\ \cline{1-1}
    all                         & 3222   & 3998   & 0.611 & 0.333  & 0.361  & 0.356  & 0.248      \\
    Airborne                    & 3222   & 357    & 0.431 & 0.0616 & 0.108  & 0.0956 & 0.0497     \\
    Airplane                    & 3222   & 867    & 0.867 & 0.609  & 0.715  & 0.683  & 0.479      \\
    Bird                        & 3222   & 151    & 0.283 & 0.0199 & 0.0371 & 0.0219 & 0.0169     \\
    Drone                       & 3222   & 36     & 0.726 & 0.778  & 0.751  & 0.794  & 0.59       \\
    Flock                       & 3222   & 22     & 1     & 0      & 0      & 0      & 0          \\
    Helicopter                  & 3222   & 2565   & 0.968 & 0.865  & 0.913  & 0.901  & 0.599      \\
    ood                         & 3222   & 0      & 0     & 0      & 0      & 0      & 0         
    \end{tabular}
\end{table}

Since the OOD class has no samples in the ID training dataset (results presented above), it achieves an AP score of \num{0}. We account for this problem by calculating the mAP score without the OOD class. These values are given in section  4 of the related paper.

==> eccv_workshop_uncertainty_ea/Chapters/results/98_details_results_baseline.tex <==
\begin{table}[]
    \begin{tabular}{llllllll}
    \cline{1-1}
    \multicolumn{1}{|l|}{Class} & Images & Labels & P      & R      & F1    & mAP@.5 & mAP@.5:.95 \\ \cline{1-1}
    all                         & 3222   & 3998   & 0.514  & 0.362  & 0.366 & 0.321  & 0.215      \\
    Airborne                    & 3222   & 357    & 0.192  & 0.157  & 0.173 & 0.0774 & 0.035      \\
    Airplane                    & 3222   & 867    & 0.686  & 0.637  & 0.66  & 0.611  & 0.417      \\
    Bird                        & 3222   & 151    & 0.0588 & 0.0927 & 0.072 & 0.0178 & 0.0118     \\
    Drone                       & 3222   & 36     & 0.757  & 0.777  & 0.767 & 0.666  & 0.478      \\
    Flock                       & 3222   & 22     & 1      & 0      & 0     & 0      & 0          \\
    Helicopter                  & 3222   & 2565   & 0.905  & 0.872  & 0.888 & 0.875  & 0.56       \\
    ood                         & 3222   & 0      & 0      & 0      & 0     & 0      & 0         
    \end{tabular}
\end{table}

Since the OOD class has no samples in the ID training dataset (results presented above), it achieves an AP score of \num{0}. We account for this problem by calculating the mAP score without the OOD class. These values are given in section  4 of the related paper.

==> eccv_workshop_uncertainty_ea/Chapters/results/99_results_table.tex <==
\begin{table}[t]
    \centering
    \caption{Results for the baseline and ME loss.
        ME loss outperforms the baseline by \SI{129}{\percent} wrt. Separability $S$.}
    \label{tab:results}
    \begin{tabular}{@{}lllllll@{}}
        \toprule
        Method           & \multicolumn{1}{c}{$S$} & \multicolumn{1}{c}{OBS} & \multicolumn{1}{c}{OFS} & \multicolumn{1}{c}{mAP@0.5} \\ \midrule
        Na\"ive Baseline & \num{0.212}             & \num{0.251}             & \num{0.184}             & \num{0.375}                 \\
        ME Loss          & \textbf{\num{0.486}}    & \textbf{\num{0.431}}    & \textbf{\num{0.556}}    & \textbf{\num{0.416}}        \\ \bottomrule
    \end{tabular}
\end{table}


%\todo{Any idea how I can reformat this table?}
%\todo{Proposal: remove thresholds, put them into the diagram description.}

==> eccv_workshop_uncertainty_ea/histograms.tex <==
\newcommand{\varBaselineSep}{0.213\:}
\newcommand{\varBaselineIdOod}{0.87\:}
\newcommand{\varBaselineOodBack}{0.35\:}
\newcommand{\varEnsemblesSep}{0.172\:}
\newcommand{\varEnsemblesIdOod}{0.301\:}
\newcommand{\varEnsemblesOodBack}{0.04\:}
\newcommand{\varMElossSep}{0.486\:}
\newcommand{\varMElossIdOod}{0.42\:}
\newcommand{\varMElossOodBack}{0.39\:}
\newcommand{\varMElossApNinetyFive}{0.248\:}
\newcommand{\varMElossApFifty}{0.356\:}
\newcommand{\vartwoDBasicSep}{0.172\:}
\newcommand{\vartwoDBasicIdOod}{0.301\:}
\newcommand{\vartwoDBasicOodBack}{0.04\:}
\newcommand{\varSepImprovement}{128.2\:}
\newcommand{\tikzBaselinePDF}{% This file was created with tikzplotlib v0.9.12.
    \begin{tikzpicture}

        \definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
        \definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
        \definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

        \begin{axis}[
                height=0.21\textwidth,
                legend cell align={left},
                legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, nodes={scale=0.75, transform shape}},
                tick pos=left,
                width=0.48\textwidth,
                x grid style={white!69.0196078431373!black},
                % xlabel={Confidence},
                xmin=0, xmax=1,
                xtick style={color=black},
                y grid style={white!69.0196078431373!black},
                ylabel={Density [\si{\percent}]},
                ylabel style={yshift=-10pt},
                ymin=-1.17296862429606, ymax=24.6323411102172,
                ytick style={color=black}
            ]
            \addplot [semithick, color0]
            table [row sep=\\] {%
                    0.0025 1.2018779342723\\0.0275 0.275430359937402\\0.0525 0.200312989045383\\0.0775 0.162754303599374\\0.1025 0.200312989045383\\0.1275 0.137715179968701\\0.1525 0.112676056338028\\0.1775 0.125195618153365\\0.2025 0.137715179968701\\0.2275 0.100156494522692\\0.2525 0.137715179968701\\0.2775 0.225352112676056\\0.3025 0.125195618153365\\0.3275 0.187793427230047\\0.3525 0.112676056338028\\0.3775 0.100156494522692\\0.4025 0.125195618153365\\0.4275 0.112676056338028\\0.4525 0.125195618153365\\0.4775 0.137715179968701\\0.5025 0.17527386541471\\0.5275 0.162754303599374\\0.5525 0.187793427230047\\0.5775 0.137715179968701\\0.6025 0.25039123630673\\0.6275 0.17527386541471\\0.6525 0.150234741784037\\0.6775 0.187793427230047\\0.7025 0.187793427230047\\0.7275 0.350547730829422\\0.7525 0.150234741784037\\0.7775 0.350547730829421\\0.8025 0.413145539906103\\0.8275 0.851330203442879\\0.8525 2.3661971830986\\0.8775 10.3787167449139\\0.9025 8.83881064162754\\0.9275 6.61032863849765\\0.9525 3.51799687010954\\0.9775 0.513302034428797\\};
            \addlegendentry{ID FG}
            \addplot [semithick, color1]
            table [row sep=\\] {%
                    0.0025 4.33734939759036\\0.0275 0.72289156626506\\0.0525 0.963855421686747\\0.0775 0.602409638554217\\0.1025 0.481927710843374\\0.1275 0.240963855421687\\0.1525 0.36144578313253\\0.1775 0.36144578313253\\0.2025 0.36144578313253\\0.2275 0.481927710843374\\0.2525 0.36144578313253\\0.2775 0.240963855421687\\0.3025 0.240963855421687\\0.3275 0.240963855421687\\0.3525 0.240963855421687\\0.3775 0.72289156626506\\0.4025 0.481927710843373\\0.4275 0.602409638554218\\0.4525 0.36144578313253\\0.4775 0.722891566265061\\0.5025 0.120481927710843\\0.5275 0.120481927710843\\0.5525 0.120481927710843\\0.5775 0.481927710843373\\0.6025 0.96385542168675\\0.6275 0.963855421686746\\0.6525 0.481927710843373\\0.6775 0.36144578313253\\0.7025 0.481927710843373\\0.7275 1.44578313253013\\0.7525 0.602409638554216\\0.7775 0.481927710843373\\0.8025 1.56626506024096\\0.8275 2.7710843373494\\0.8525 3.73493975903616\\0.8775 4.57831325301204\\0.9025 3.49397590361445\\0.9275 3.01204819277108\\0.9525 1.08433734939759\\0.9775 0\\};
            \addlegendentry{OOD}
            \addplot [semithick, color2]
            table [row sep=\\] {%
                    0.0025 23.4593724859212\\0.0275 1.81818181818182\\0.0525 1.02976669348351\\0.0775 0.901045856798069\\0.1025 0.707964601769912\\0.1275 0.466613032984714\\0.1525 0.498793242156074\\0.1775 0.386162510056315\\0.2025 0.482703137570394\\0.2275 0.289621882542237\\0.2525 0.370072405470635\\0.2775 0.241351568785197\\0.3025 0.321802091713597\\0.3275 0.176991150442478\\0.3525 0.193081255028158\\0.3775 0.241351568785197\\0.4025 0.193081255028158\\0.4275 0.176991150442478\\0.4525 0.160901045856798\\0.4775 0.273531777956557\\0.5025 0.386162510056315\\0.5275 0.160901045856798\\0.5525 0.225261464199517\\0.5775 0.209171359613837\\0.6025 0.144810941271119\\0.6275 0.353982300884955\\0.6525 0.434432823813354\\0.6775 0.160901045856798\\0.7025 0.305711987127916\\0.7275 0.402252614641997\\0.7525 0.289621882542236\\0.7775 0.482703137570394\\0.8025 0.209171359613837\\0.8275 0.418342719227675\\0.8525 0.884955752212393\\0.8775 1.22284794851166\\0.9025 0.820595333869669\\0.9275 0.337892196299276\\0.9525 0.144810941271118\\0.9775 0.0160901045856799\\};
            \addlegendentry{ID BG}
        \end{axis}

    \end{tikzpicture}
}
\newcommand{\tikzEnsemblesPDF}{% This file was created with tikzplotlib v0.9.12.
    \begin{tikzpicture}

        \definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
        \definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
        \definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

        \begin{axis}[
                height=0.4\textwidth,
                legend cell align={left},
                legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, nodes={scale=0.75, transform shape}},
                tick pos=left,
                width=0.48\textwidth,
                x grid style={white!69.0196078431373!black},
                xlabel={Confidence},
                xmin=0, xmax=1,
                xtick style={color=black},
                y grid style={white!69.0196078431373!black},
                ylabel={Density [\si{\percent}]},
                ymin=-1.27380952380952, ymax=26.75,
                ytick style={color=black}
            ]
            \addplot [semithick, color0]
            table [row sep=\\] {%
                    0.0025 1.42724170027924\\0.0275 0.297859137449581\\0.0525 0.248215947874651\\0.0775 0.198572758299721\\0.1025 0.260626745268384\\0.1275 0.173751163512256\\0.1525 0.136518771331058\\0.1775 0.223394353087186\\0.2025 0.124107973937326\\0.2275 0.136518771331058\\0.2525 0.173751163512256\\0.2775 0.173751163512256\\0.3025 0.111697176543593\\0.3275 0.136518771331058\\0.3525 0.124107973937326\\0.3775 0.161340366118523\\0.4025 0.0620539869686627\\0.4275 0.148929568724791\\0.4525 0.0620539869686627\\0.4775 0.136518771331058\\0.5025 0.136518771331058\\0.5275 0.14892956872479\\0.5525 0.111697176543593\\0.5775 0.124107973937325\\0.6025 0.173751163512256\\0.6275 0.136518771331058\\0.6525 0.161340366118523\\0.6775 0.260626745268383\\0.7025 0.161340366118523\\0.7275 0.310269934843315\\0.7525 0.260626745268383\\0.7775 0.359913124418244\\0.8025 0.533664287930499\\0.8275 0.93080980452994\\0.8525 3.67359602854485\\0.8775 9.71765435929258\\0.9025 8.05460750853242\\0.9275 5.33664287930499\\0.9525 3.6984176233323\\0.9775 1.19143654979833\\};
            \addlegendentry{ID FG}
            \addplot [semithick, color1]
            table [row sep=\\] {%
                    0.0025 2.38095238095238\\0.0275 1.19047619047619\\0.0525 0.634920634920635\\0.0775 0.873015873015873\\0.1025 0.476190476190476\\0.1275 0.873015873015872\\0.1525 0.555555555555556\\0.1775 0.476190476190476\\0.2025 0.634920634920635\\0.2275 0.634920634920635\\0.2525 0.396825396825396\\0.2775 1.03174603174603\\0.3025 1.03174603174603\\0.3275 1.74603174603174\\0.3525 6.90476190476191\\0.3775 10.5555555555555\\0.4025 3.09523809523809\\0.4275 0.714285714285715\\0.4525 0.0793650793650793\\0.4775 0\\0.5025 0\\0.5275 0.158730158730159\\0.5525 0.238095238095238\\0.5775 0.0793650793650793\\0.6025 0.158730158730159\\0.6275 0.158730158730159\\0.6525 0.238095238095238\\0.6775 0.238095238095238\\0.7025 0.0793650793650793\\0.7275 0.476190476190478\\0.7525 0.0793650793650793\\0.7775 0.396825396825396\\0.8025 0.634920634920634\\0.8275 0.396825396825396\\0.8525 0.873015873015876\\0.8775 0.317460317460317\\0.9025 0.714285714285714\\0.9275 0.317460317460317\\0.9525 0.158730158730159\\0.9775 0\\};
            \addlegendentry{OOD}
            \addplot [semithick, color2]
            table [row sep=\\] {%
                    0.0025 25.4761904761905\\0.0275 2.42857142857143\\0.0525 1.13095238095238\\0.0775 0.857142857142857\\0.1025 0.55952380952381\\0.1275 0.464285714285714\\0.1525 0.345238095238095\\0.1775 0.333333333333333\\0.2025 0.321428571428572\\0.2275 0.440476190476191\\0.2525 0.345238095238095\\0.2775 0.309523809523809\\0.3025 0.166666666666667\\0.3275 0.214285714285714\\0.3525 0.25\\0.3775 0.273809523809524\\0.4025 0.25\\0.4275 0.273809523809524\\0.4525 0.238095238095238\\0.4775 0.166666666666667\\0.5025 0.19047619047619\\0.5275 0.25\\0.5525 0.154761904761905\\0.5775 0.19047619047619\\0.6025 0.166666666666667\\0.6275 0.154761904761905\\0.6525 0.226190476190476\\0.6775 0.297619047619047\\0.7025 0.178571428571428\\0.7275 0.214285714285715\\0.7525 0.142857142857143\\0.7775 0.25\\0.8025 0.297619047619047\\0.8275 0.19047619047619\\0.8525 0.678571428571431\\0.8775 0.797619047619047\\0.9025 0.392857142857143\\0.9275 0.154761904761905\\0.9525 0.226190476190476\\0.9775 0\\};
            \addlegendentry{ID BG}
        \end{axis}

    \end{tikzpicture}
}
\newcommand{\tikzMElossPDF}{% This file was created with tikzplotlib v0.9.12.
    \begin{tikzpicture}

        \definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
        \definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
        \definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

        \begin{axis}[
                height=0.21\textwidth,
                legend cell align={left},
                legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, nodes={scale=0.75, transform shape}},
                tick pos=left,
                width=0.48\textwidth,
                x grid style={white!69.0196078431373!black},
                xlabel={Confidence},
                xmin=0, xmax=1,
                xtick style={color=black},
                y grid style={white!69.0196078431373!black},
                ylabel={Density [\si{\percent}]},
                ylabel style={yshift=-10pt},
                ymin=-1.53882653526782, ymax=32.3153572406241,
                ytick style={color=black}
            ]
            \addplot [semithick, color0]
            table [row sep=\\] {%
                    0.0025 2.59563615755171\\0.0275 0.612071408330972\\0.0525 0.408047605553981\\0.0775 0.453386228393313\\0.1025 0.487390195522811\\0.1275 0.476055539812978\\0.1525 0.328705015585152\\0.1775 0.260697081326155\\0.2025 0.170019835647492\\0.2275 0.28336639274582\\0.2525 0.147350524227826\\0.2775 0.226693114196656\\0.3025 0.215358458486824\\0.3275 0.124681212808161\\0.3525 0.0793425899688298\\0.3775 0.147350524227826\\0.4025 0.136015868517994\\0.4275 0.170019835647492\\0.4525 0.102011901388495\\0.4775 0.147350524227827\\0.5025 0.20402380277699\\0.5275 0.136015868517994\\0.5525 0.147350524227826\\0.5775 0.136015868517994\\0.6025 0.181354491357326\\0.6275 0.215358458486823\\0.6525 0.170019835647492\\0.6775 0.249362425616322\\0.7025 0.351374327004817\\0.7275 0.532728818362144\\0.7525 0.974780391045621\\0.7775 1.60952111079626\\0.8025 3.77444035137432\\0.8275 5.92802493624256\\0.8525 7.40153017852085\\0.8775 4.48852366109379\\0.9025 2.7996599603287\\0.9275 2.18758855199773\\0.9525 0.895437801076791\\0.9775 0.0453386228393314\\};
            \addlegendentry{ID FG}
            \addplot [semithick, color1]
            table [row sep=\\] {%
                    0.0025 0\\0.0275 1.35593220338983\\0.0525 0.677966101694915\\0.0775 0.677966101694915\\0.1025 0\\0.1275 0.677966101694915\\0.1525 0\\0.1775 0\\0.2025 0.677966101694915\\0.2275 0\\0.2525 0.677966101694915\\0.2775 1.35593220338983\\0.3025 2.03389830508475\\0.3275 1.35593220338983\\0.3525 3.38983050847458\\0.3775 10.1694915254237\\0.4025 16.271186440678\\0.4275 0.677966101694916\\0.4525 0\\0.4775 0\\0.5025 0\\0.5275 0\\0.5525 0\\0.5775 0\\0.6025 0\\0.6275 0\\0.6525 0\\0.6775 0\\0.7025 0\\0.7275 0\\0.7525 0\\0.7775 0\\0.8025 0\\0.8275 0\\0.8525 0\\0.8775 0\\0.9025 0\\0.9275 0\\0.9525 0\\0.9775 0\\};
            \addlegendentry{OOD}
            \addplot [semithick, color2]
            table [row sep=\\] {%
                    0.0025 30.7765307053563\\0.0275 2.52577789944338\\0.0525 1.18258965234054\\0.0775 0.722693676430331\\0.1025 0.565745049730815\\0.1275 0.386896614654621\\0.1525 0.324847157587371\\0.1775 0.310247285336253\\0.2025 0.208048179578429\\0.2275 0.215348115703988\\0.2525 0.259147732457341\\0.2775 0.233597956017885\\0.3025 0.182498403138973\\0.3275 0.182498403138972\\0.3525 0.211698147641208\\0.3775 0.105849073820604\\0.4025 0.0875992335067067\\0.4275 0.0474495848161329\\0.4525 0.0693493931928095\\0.4775 0.0620494570672507\\0.5025 0.0547495209416917\\0.5275 0.0547495209416917\\0.5525 0.0547495209416917\\0.5775 0.0510995528789123\\0.6025 0.0693493931928098\\0.6275 0.0547495209416917\\0.6525 0.0547495209416917\\0.6775 0.0693493931928095\\0.7025 0.0510995528789123\\0.7275 0.0583994890044714\\0.7525 0.124098914134501\\0.7775 0.149648690573957\\0.8025 0.175198467013413\\0.8275 0.120448946071722\\0.8525 0.0948991696322661\\0.8775 0.0437996167533534\\0.9025 0.0364996806277945\\0.9275 0.0218998083766767\\0.9525 0\\0.9775 0\\};
            \addlegendentry{ID BG}
        \end{axis}

    \end{tikzpicture}
}
\newcommand{\tikztwoDBasicPDF}{% This file was created with tikzplotlib v0.9.12.
    \begin{tikzpicture}

        \definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
        \definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
        \definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

        \begin{axis}[
                height=0.4\textwidth,
                legend cell align={left},
                legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, nodes={scale=0.75, transform shape}},
                tick pos=left,
                width=0.48\textwidth,
                x grid style={white!69.0196078431373!black},
                xlabel={Confidence},
                xmin=0, xmax=1,
                xtick style={color=black},
                y grid style={white!69.0196078431373!black},
                ylabel={Probability},
                ymin=-1.27380952380952, ymax=26.75,
                ytick style={color=black}
            ]
            \addplot [semithick, color0]
            table [row sep=\\] {%
                    0.0025 1.42724170027924\\0.0275 0.297859137449581\\0.0525 0.248215947874651\\0.0775 0.198572758299721\\0.1025 0.260626745268384\\0.1275 0.173751163512256\\0.1525 0.136518771331058\\0.1775 0.223394353087186\\0.2025 0.124107973937326\\0.2275 0.136518771331058\\0.2525 0.173751163512256\\0.2775 0.173751163512256\\0.3025 0.111697176543593\\0.3275 0.136518771331058\\0.3525 0.124107973937326\\0.3775 0.161340366118523\\0.4025 0.0620539869686627\\0.4275 0.148929568724791\\0.4525 0.0620539869686627\\0.4775 0.136518771331058\\0.5025 0.136518771331058\\0.5275 0.14892956872479\\0.5525 0.111697176543593\\0.5775 0.124107973937325\\0.6025 0.173751163512256\\0.6275 0.136518771331058\\0.6525 0.161340366118523\\0.6775 0.260626745268383\\0.7025 0.161340366118523\\0.7275 0.310269934843315\\0.7525 0.260626745268383\\0.7775 0.359913124418244\\0.8025 0.533664287930499\\0.8275 0.93080980452994\\0.8525 3.67359602854485\\0.8775 9.71765435929258\\0.9025 8.05460750853242\\0.9275 5.33664287930499\\0.9525 3.6984176233323\\0.9775 1.19143654979833\\};
            \addlegendentry{ID FG}
            \addplot [semithick, color1]
            table [row sep=\\] {%
                    0.0025 2.38095238095238\\0.0275 1.19047619047619\\0.0525 0.634920634920635\\0.0775 0.873015873015873\\0.1025 0.476190476190476\\0.1275 0.873015873015872\\0.1525 0.555555555555556\\0.1775 0.476190476190476\\0.2025 0.634920634920635\\0.2275 0.634920634920635\\0.2525 0.396825396825396\\0.2775 1.03174603174603\\0.3025 1.03174603174603\\0.3275 1.74603174603174\\0.3525 6.90476190476191\\0.3775 10.5555555555555\\0.4025 3.09523809523809\\0.4275 0.714285714285715\\0.4525 0.0793650793650793\\0.4775 0\\0.5025 0\\0.5275 0.158730158730159\\0.5525 0.238095238095238\\0.5775 0.0793650793650793\\0.6025 0.158730158730159\\0.6275 0.158730158730159\\0.6525 0.238095238095238\\0.6775 0.238095238095238\\0.7025 0.0793650793650793\\0.7275 0.476190476190478\\0.7525 0.0793650793650793\\0.7775 0.396825396825396\\0.8025 0.634920634920634\\0.8275 0.396825396825396\\0.8525 0.873015873015876\\0.8775 0.317460317460317\\0.9025 0.714285714285714\\0.9275 0.317460317460317\\0.9525 0.158730158730159\\0.9775 0\\};
            \addlegendentry{OOD}
            \addplot [semithick, color2]
            table [row sep=\\] {%
                    0.0025 25.4761904761905\\0.0275 2.42857142857143\\0.0525 1.13095238095238\\0.0775 0.857142857142857\\0.1025 0.55952380952381\\0.1275 0.464285714285714\\0.1525 0.345238095238095\\0.1775 0.333333333333333\\0.2025 0.321428571428572\\0.2275 0.440476190476191\\0.2525 0.345238095238095\\0.2775 0.309523809523809\\0.3025 0.166666666666667\\0.3275 0.214285714285714\\0.3525 0.25\\0.3775 0.273809523809524\\0.4025 0.25\\0.4275 0.273809523809524\\0.4525 0.238095238095238\\0.4775 0.166666666666667\\0.5025 0.19047619047619\\0.5275 0.25\\0.5525 0.154761904761905\\0.5775 0.19047619047619\\0.6025 0.166666666666667\\0.6275 0.154761904761905\\0.6525 0.226190476190476\\0.6775 0.297619047619047\\0.7025 0.178571428571428\\0.7275 0.214285714285715\\0.7525 0.142857142857143\\0.7775 0.25\\0.8025 0.297619047619047\\0.8275 0.19047619047619\\0.8525 0.678571428571431\\0.8775 0.797619047619047\\0.9025 0.392857142857143\\0.9275 0.154761904761905\\0.9525 0.226190476190476\\0.9775 0\\};
            \addlegendentry{ID BG}
        \end{axis}

    \end{tikzpicture}
}
\newcommand{\tabBaseline}{\begin{tabular}{rrrr}
        \hline
        separability & ood\_back\_thres & id\_ood\_thres & ap50 \\
        \hline
        0.213        & 0.35             & 0.87           & nan  \\
        \hline
    \end{tabular}}
\newcommand{\tabEnsembles}{\begin{tabular}{rrrr}
        \hline
        separability & ood\_back\_thres & id\_ood\_thres & ap50 \\
        \hline
        0.172        & 0.04             & 0.301          & nan  \\
        \hline
    \end{tabular}}
\newcommand{\tabMEloss}{\begin{tabular}{rrrr}
        \hline
        separability & ood\_back\_thres & id\_ood\_thres & ap50  \\
        \hline
        0.486        & 0.39             & 0.42           & 0.356 \\
        \hline
    \end{tabular}}
\newcommand{\tabtwoDBasic}{\begin{tabular}{rrrr}
        \hline
        separability & ood\_back\_thres & id\_ood\_thres & ap50 \\
        \hline
        0.172        & 0.04             & 0.301          & nan  \\
        \hline
    \end{tabular}}
\newcommand{\tabGlobal}{\begin{tabular}{lrr}
        \hline
        Method   & Separability & ap50  \\
        \hline
        Baseline & 0.213        & nan   \\
        ME Loss  & 0.486        & 0.356 \\
        \hline
    \end{tabular}}

